D3: Deep Deconvolution Deblurring for Natural Images

In this paper, we propose to reformulate the blind image deblurring task to directly learn an inverse of the degradation model represented by a deep linear network. We introduce Deep Identity Learning (DIL), a novel learning strategy that includes a dedicated regularization term based on the properties of linear systems, to exploit the identity relation between the degradation and inverse degradation models. The salient aspect of our proposed framework is it neither relies on a deblurring dataset nor a single input blurry image (e.g. Polyblur, a self-supervised method). This framework detours the typical degradation kernel estimation step involved in most of the existing blind deblurring solutions by the proposition of our Random Kernel Gallery (RKG) dataset. The proposed approach extends our previous Image Super-Resolution (ISR) work, NSSR-DIL, to the image deblurring task. In this work, we updated the regularization term in DIL based on Fourier transform properties of the identity relation, to deliver robust performance across a wide range of degradations. Besides the regularization term, we provide an explicit and compact representation of the learned deep linear network in a matrix form, called Deep Restoration Kernel (DRK) to perform image restoration. Our experiments show that the proposed method outperforms both traditional and deep learning based deblurring methods, with at least an order of 100 lesser computational resources. The D3 model, both LCNN & DRK, can be effortlessly extended to the Image Super-Resolution (ISR) task as well to restore the low-resolution images with fine details. The D3 model and its kernel form representation (DRK) are lightweight yet robust and restore the blurry input in a fraction of a second.

==> storeroom.tex <==

 %  \item We propose a novel learning function i.e. DIL with a dedicated regularization term to effectively learn an inverse degradation model based on identity system properties. 
    % \item The proposed blind deblurring method bypasses the typical kernel estimation step by the generated robust RKG dataset. 

% Instead of the data-driven or self-supervised approaches for low-level vision restoration tasks, in our previous work \cite{nssrdil}, we presented a computationally efficient Null-Shot ISR approach called ``Null-Shot Image Super-Resolution Using Deep Identity Learning (NSSR-DIL)". In this work, we introduced a novel learning strategy called “Deep Identity Learning” (DIL), that exploits the identity relation between the degradation model $K$ and its inverse $K^{-1}$ i.e., the ISR model.\\

%Further, we provide the mathematical representation of the raw matrix values of the DRK matrix using the Gaussian mixture model and Sum of Sine functions. 


%by using the key ideas of degradation model representation, linear restoration model and learning objective based on identity relation with improvised regularization term. 
% We defined the degradation model by a set of kernels, referred to as the Random Kernel Gallery (RKG) dataset. Later, we learn the degradation model characterized by a custom shallow Convolutional Neural Network (CNN), with no activation functions referred to as Linear-CNN (L-CNN). The linear model was considered to comply with the linear definition of the convolution operation. L-CNN was trained with DIL objective using RKG dataset to form the inverse degradation model i.e., the ISR model. Unlike existing self-supervised zero-shot ISR frameworks \cite{zssr}, \cite{dbpi}, and \cite{dualsr} the proposed NSSR-DIL model is image independent and doesn't require LR-HR pair or LR image data at any stage of the ISR task learning. \\
% In recent literature, it is observed that most of the works were leaning towards addressing the strong motion and non-uniform blur \cite{li2023self,ren2020neural, kupyn2018deblurgan, xy, IFFS}. However, very little attention was paid to the most common and practical use case where the blur is small i.e. mild blur that is often present in real images which degrades the image quality. Mild blur can be harmful to the performance of other image processing tasks, such as super-resolution. These tasks often rely on sharp images to produce accurate results. The works \cite{polyblur, zhu2011restoration}, detached from the mainstream deblurring methods and were proposed solutions towards addressing the mild blur. For instance, Polyblur \cite{polyblur} is a blind and self-supervised approach that uses polynomial functions to restore image details blurred by mild camera shake or motion blur supporting real-time applications. It estimates the blur kernel of the image by analyzing the distribution of the gradient in the image and then applies the kernel multiple times, based on the severity of the blur.\\
% The major limitation, especially in non-blind methods, is the error-free assumption on the blur kernel. In practice, the estimated blur kernel is prone to error. Even the slight deviation in the estimated blur kernel leads to ill-posedness of the problem as it results in great mismatch of the deconvolution kernel followed by the notable artefacts in the deblurred image \cite{partialdeconv, ji2011robust, li2023self}. In case of the blind deblurring methods, the extensive dependency on datasets for prior information could limit their generalization ability.  \\
% While promising, the present State-of-the-Art (SotA) image deblurring methods grapple with generalization issues in memory-constrained environments due to their sizable footprint.
% Despite vigorous research efforts, the existing deblurring algorithms still exhibit the inverse correlation between the accuracy and the computational efficiency \cite{polyblur, chiang2020deploying, 1shot}.
% Besides these drawbacks, the present State-of-the-Art (SotA) image deblurring methods employ DL techniques using a large amount of image data with heavy computational and time complexities.

% On other hand, the methods DeblurGAN and XYDeblur are supervised and USRNet is an unsupervised data-driven deblurring method. 
